Transition-Aware Multi-Activity Knowledge Tracing

Accurate modeling of student knowledge is essential for large-scale online learning systems that are increasingly used for student training. Knowledge tracing aims to model student knowledge state given the student's sequence of learning activities. Modern Knowledge tracing (KT) is usually formulated as a supervised sequence learning problem to predict students' future practice performance according to their past observed practice scores by summarizing student knowledge state as a set of evolving hidden variables. Because of this formulation, many current KT solutions are not fit for modeling student learning from non-assessed learning activities with no explicit feedback or score observation (e.g., watching video lectures that are not graded). Additionally, these models cannot explicitly represent the dynamics of knowledge transfer among different learning activities, particularly between the assessed (e.g., quizzes) and non-assessed (e.g., video lectures) learning activities. In this paper, we propose Transition-Aware Multi-activity Knowledge Tracing (TAMKOT), which models knowledge transfer between learning materials, in addition to student knowledge, when students transition between and within assessed and non-assessed learning materials. TAMKOT is formulated as a deep recurrent multi-activity learning model that explicitly learns knowledge transfer by activating and learning a set of knowledge transfer matrices, one for each transition type between student activities. Accordingly, our model allows for representing each material type in a different yet transferrable latent space while maintaining student knowledge in a shared space. We evaluate our model on three real-world publicly available datasets and demonstrate TAMKOT's capability in predicting student performance and modeling knowledge transfer.

==> 5.7-resource.tex <==
\begin{figure*}[!ht]
   \vspace{-5pt}
    \centering
    \subfigure{
    \includegraphics[width=0.3\textwidth]{figures/morf_tsne_L.pdf}}
    \subfigure{
    \includegraphics[width=0.6\textwidth]{figures/2022-CIKM-MTDKT-tsne_titile_L.pdf}}   
    \vspace{-10pt}
    \caption{Within-Type concept analysis. Cluster results of MORF video lectures (left) and table of video lectures' titles(right).
    Lectures clustered in the same group are labeled in the same color and are in the same group are in the same block.}
    \label{fig:learning_resorce_analysis_lecture}
    \vspace{-10pt}
\end{figure*}

\begin{figure*}[!ht]
   \vspace{-5pt}
    \centering
    \subfigure{
    \includegraphics[width=0.3\textwidth]{figures/morf_tsne_Q_L.pdf}}
    \subfigure{
    \includegraphics[width=0.6\textwidth]{figures/2022-CIKM-MTDKT-tsne_titile_QL.pdf}}
   \vspace{-10pt}
    \caption{Between-Type concept analysis. Cluster results of MORF video lectures and assignments (left) and table of video lectures and assignments' titles (right). Lectures and assignments clustered in the same group are labeled in the same color and are in the same block. We use "." and "x" for video lectures and assignments, respectively.} 
    \label{fig:learning_resorce_analysis_quiz_lecture}
   \vspace{-10pt}
\end{figure*}



In this section, we would like to validate if TAMKOT could discover meaningful latent concepts for each learning material.
% Since the MORF dataset includes learning material contents, we conduct the latent concept analysis on this dataset.
We perform the latent concept analysis on the MORF dataset.
Since both Junyi and Ednet have many learning materials, we cannot present the visualization of these two datasets due to the page limits.
We evaluate the discovered latent concepts in two aspects: 1) within-type concept analysis, which compares the latent concepts of the same learning material type, and 2) between-type concept analysis, which compares the latent concepts of learning materials in different material types (assessed vs. non-assessed). 
% We use the textual content information of video lectures and assignments as the representation of their concepts to validate if our discovered latent concepts are interpretable.
% We expect that two learning materials should share similar latent concepts if they have similar textual contents. 


\textbf{Within-Type Concept Analysis.}
Firstly, we apply Spectral Clustering to cluster the video lectures based on their latent concept representations in matrix ${A}^l$ and find 8 clusters.
Then, t-SNE~\cite{van2008visualizing} is used to project each high-dimensional video lecture embedding in a two-dimensional point for visualization. 
We use two-dimensional scatter plot and show the results in Figure~\ref{fig:learning_resorce_analysis_lecture}, where the video lectures from the same cluster are labeled in the same color.
The ground truth video lecture concept is not provided in the MORF dataset, but we have access to the title of each video lecture.
On the right side of Figure~\ref{fig:learning_resorce_analysis_lecture}, we show these titles, each block represents a cluster of video lectures in the spectral clustering results.

From clustering results, we can see that some video lectures from the same weeks are clustered together. 
For example, four videos of week 4 are clustered in the same cluster, their titles reveal that these four video lectures are related to the same topic: ``knowledge tracing''.
This shows the proposed method TAMKOT can discover meaningful latent concepts for learning materials.
In addition, some weeks of video lectures are clustered in several different groups. 
For example, six videos of week 6 are clustered into five different clusters.
One possible reason could be because the topic of week 6 is about ``visualization'', which may be relevant to all content in the course. For example, it can be a scatter plot introduced by using a clustering example discussed in W6 V1.
% This also indicates that our TAMKOT can learn reasonable underlying concepts.

% We use different colors to indicate different clusters
% We firstly employ the Latent Dirichlet Analysis (LDA) to discover latent topics for each video lecture from its textual contents. 
% Then, we apply Spectral Clustering to cluster the video lectures once based on their LDA topics and another time based on the embedding matrix ${A}^l$. 
% The two clustering results are shown in Figure~\ref{fig:learning_resorce_analysis_lecture}. 
% We use different colors to indicate different clusters based on LDA topics.
% As shown in~\ref{fig: LDA_cluster_lecture}, we find 8 clusters based on LDA topics. 
% The clusters achieved based on embedding matrix ${A}^{l}$ are shown in~\ref{fig: TAMKOT_cluster_lecture}. 
% We can see that some video lectures from the same weeks are clustered together. 
% For example, three videos of week 6 are in the same cluster (cluster 5) as shown in Figure~\ref{fig: TAMKOT_cluster_lecture}. 
% In addition, four video lectures in week 7 are also clustered into the same group (cluster 5), although these 4 video lectures have different topics discovered by LDA.
% Looking at the MDTKD clusters in Figure~\ref{fig: TAMKOT_cluster_lecture}, we see that the learning material embeddings discovered by MDTKD also contain some topic-related information.   
% For example, the W3 V5, W6 V2, and W8 V1 are clustered together in cluster 8, although they are from three different weeks. 


\textbf{Between-Type Concept Analysis.} 
% TAMKOT models the embedding of assessed and non-assessed learning materials into different embedding matrices, that could have different embedding sizes. 
TAMKOT models different types of learning materials with different embedding matrices, the embedding sizes could be different for assessed and non-assessed learning materials.
Thus, we cannot directly perform cluster on latent concept representations in $\mathbold{A}^q$ and $\mathbold{A}^l$ for between-type concept analysis.
% Instead, we utilize the latent representations of learning materials at the hidden transfer layer level.
Instead, we leverage the weight matrices $\mathbold{V}_{iQ}$ and $\mathbold{V}_{iL}$ of the input gate for mapping the materials' latent concept representation into the same space.
Since $\mathbold{V}_{iQ}$ is the weight matrix of mapping $[\mathbold{q}_t \oplus \mathbold{r}_t]$ (the concatenation of question representation and student performance representation) to the hidden knowledge transfer layer, 
we partially mask $\mathbold{V}_{iQ}$ to ignore the information on student performance and denote the masked weight matrix as $\mathbold{\widehat{W}}_{iQ}$.
Finally, we calculate $\mathbold{\tilde{A}}^q=\mathbold{A}^q \mathbold{\widehat{W}}_{iQ}$ and $\mathbold{\tilde{A}}^l = {A}^l \mathbold{V}_{iL}$.
By doing so, $\mathbold{\tilde{A}}^q$ and $\mathbold{\tilde{A}}^l$ represent video lecture and assignment in the same latent space and are comparable.
Similarly, we apply the Spectral Clustering on $\mathbold{\tilde{A}}^q$ and $\mathbold{\tilde{A}}^l$ and find 8 clusters. 
The left side of figure~\ref{fig:learning_resorce_analysis_quiz_lecture} shows the clustering results, t-SNE is used to visualize video lectures and assignments in two-dimensional.
The table on the right side of figure~\ref{fig:learning_resorce_analysis_quiz_lecture} shows the title of learning materials, video lectures, and assignments that are in the same block from the same cluster.
% For example, four videos of week 4 are clustered in the same cluster, their titles reveal that all these four video lectures are related to the same topic, ``knowledge inference''.

First, we observe that the mapped representations can capture interpretable learning material concepts as well.
Some video lectures from the same weeks are clustered together.
As we can see, four videos of week 4 (the example we mentioned in the within-type analysis) are still clustered in the same group.
On the other hand, we find that all assignments are distributed in 2 clusters.
One possible reason for this result could be that each assignment contains questions related to multiple video lectures. 
This complicates the discovered concepts in each assignment, making it difficult for TAMKOT to discover to tease them out.
% Moreover, comparing the 2-D points of learning materials in within-type and between-type t-SNE figures, we observe that they are more close-knit in between-type results.
% This means that, while our model captures various learning material concepts, but in the latent space of transferring knowledge, different concepts may be similar and have the same help in improving knowledge.



% we calculate $\mathbold{A}^q \mathbold{V}_{iQ}$ and ${A}^l \mathbold{V}_{iQ}$ and apply the Spectral Clustering.
% TAMKOT models the embedding of assessed and non-assessed learning materials into different embedding matrices, that could have different embedding sizes. 
% Thus, we cannot directly use the embedding matrices $\mathbold{A}^q$ and $\mathbold{A}^l$ to do clustering on both material types together. 
% Instead, we calculate $\mathbold{A}^q \mathbold{V}_{iQ}$ and ${A}^l \mathbold{V}_{iQ}$ and apply the Spectral Clustering.
% % We mask the weight for student performance in $\mathbold{V}_{iQ}$ as 0 to make $\mathbold{A}^q \mathbold{V}_{iQ}$ an assignments-only matrix. 
% Since the $\mathbold{V}_{iQ}$ is the input gate weight matrix of $[\mathbold{q}_t \oplus \mathbold{r}_t]$ (the concatenation of question embedding and outcome embedding) , we partially mask the weight matrix $\mathbold{V}_{iQ}$ as $0$ for the part of $\mathbold{r}_t$.
% As the result, we build the TAMKOT clusters and show them in figure \ref{fig: TAMKOT_cluster_lecturequiz}.
% Similarly, we apply the Spectral Clustering on the LDA topics of assignments and video lectures, we find 8 clusters and the clustering result is shown in Figure~\ref{fig: LDA_cluster_lecturequiz}.
% As shown in figure~\ref{fig: TAMKOT_cluster_lecturequiz}, in TAMKOT clustering results, we still can find that some video lectures from the same weeks are clustered together. For example, week 7's videos 1, 2, and 3 are clustered together in figure~\ref{fig: TAMKOT_cluster_lecturequiz} cluster 2.
% On the other hand, TAMKOT can also discover the topic similarities as LDA does, both for assignments and video lectures. For example, W4 V1, W4 V2, and W4 V3 in TAMKOT cluster 8 are all in LDA topic cluster 1. 

